HoloAssist: an Egocentric Human Interaction Dataset for Interactive AI Assistants in the Real World

Building an interactive AI assistant that can perceive, reason, and collaborate with humans in the real world has been a long-standing pursuit in the AI community. This work is part of a broader research effort to develop intelligent agents that can interactively guide humans through performing tasks in the physical world. As a first step in this direction, we introduce HoloAssist, a large-scale egocentric human interaction dataset, where two people collaboratively complete physical manipulation tasks. The task performer executes the task while wearing a mixed-reality headset that captures seven synchronized data streams. The task instructor watches the performer's egocentric video in real time and guides them verbally. By augmenting the data with action and conversational annotations and observing the rich behaviors of various participants, we present key insights into how human assistants correct mistakes, intervene in the task completion procedure, and ground their instructions to the environment. HoloAssist spans 166 hours of data captured by 350 unique instructor-performer pairs. Furthermore, we construct and present benchmarks on mistake detection, intervention type prediction, and hand forecasting, along with detailed analysis. We expect HoloAssist will provide an important resource for building AI assistants that can fluidly collaborate with humans in the real world. Data can be downloaded at https://holoassist.github.io/.

==> tabs/action_anticipation.tex <==
\begin{table*}[h]
\centering
\setlength{\tabcolsep}{4pt} 
\adjustbox{width=\linewidth}{
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Modalities} & \multicolumn{3}{c|}{All Class Accuracy} & \multicolumn{3}{c|}{Head Class Accuracy} & \multicolumn{3}{c}{Tail Class Accuracy} \\ 
 & Top1 / 5 Act & Top1 / 5 Verb & Top1 / 5 Noun & Top1 / 5 Action & Top1 / 5 Verb & Top1 / 5 Noun & Top1 / 5 Action & Top1 / 5 Verb & Top1 / 5 Noun \\ \midrule
RGB & 4.10 / 18.20 & 15.17 / 56.23 & 19.06/39.83 & 4.57 / 20.29 & 16.26 / 60.25 & 20.44 / 42.44 & 0.00 / 0.00 & 5.64 / 21.20 & 7.01 / 17.09 \\ \midrule
Depth & 2.76 / 12.04 & 14.69 / 52.26 & 11.13 / 25.56 & 3.08 / 13.45 & 15.69 / 56.11 & 12.04 / 27.38 
& 0.00 / 0.00 & 6.12 / 19.23 & 3.32 / 9.97 \\
R+D & 3.76 / 16.61 & 15.00 / 53.13 & 17.30 / 37.69 & 4.20 / 18.53 & 16.00 / 57.19 & 18.85 / 40.28 & 0.00 / 0.02 & 6.47 / 18.36 & 4.02 / 15.56 \\ \midrule
Hands &  2.45 / 10.96 & 13.83 / 51.85 & 13.66 / 24.45 & 2.73 / 12.20 & 14.87 / 55.37 & 14.85 / 26.58 & 0.00 / 0.02 & 4.79 / 21.20 & 3.25 / 5.81  \\
R+H & 3.73 / 15.15 
& 13.34 / 51.80 & 18.06 / 35.81 
& 4.16 / 16.89 & 14.26 / 55.50 & 19.56 / 38.28 & 0.00 / 0.00 & 5.30 / 19.49 & 4.96 / 14.36  \\
\midrule
R+D+H & 2.69 / 11.69 & 14.29 / 51.96 & 13.58 / 28.70 & 3.00 / 13.06 & 15.32 / 55.76 & 14.75 / 30.93 & 0.00 / 0.00 & 5.42 / 19.41 & 3.50 / 9.62 \\
\midrule\midrule
RGB (Pt) & 5.00 / 20.68 & 15.70 / 55.19 & 21.96 / 49.21 & 5.57 / 23.01 & 16.72 / 59.21 & 22.95 / 51.38 & 0.00 / 0.04 & 6.84 / 20.17 & 13.33 / 30.26 \\ \bottomrule
\end{tabular}}\caption{{Action anticipation benchmark results with TimesFormer} The TimeSformer~\cite{timesformer} models in the forecast 1 second into future. Similar to action recognition, we notice that adding hands information (\texttt{R+H}) outperforms the baseline \texttt{RGB} models and depth hurts the prediction performance. The pretrained RGB model (\texttt{RGB(Pt)}) achieves 9.65\% and 30.82\% top-1 and 5 accuracies. In general, the tail classes are very challenging with less 1\% accuracy across the models. } \label{tab:act_anticipation} 
\end{table*}



==> tabs/action_recognition.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{4pt} 
\adjustbox{width=\linewidth}{
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|ccc|ccc|ccc@{}}
\toprule
\multirow{2}{*}{Mods.}& \multicolumn{3}{c|}{All Classes Accuracy}& \multicolumn{3}{c|}{Head Classes Accuracy} & \multicolumn{3}{c}{Tail Classes Accuracy}               \\
 & Top1 / 5 Act  & Top1 / 5 Verb  & Top1 / 5 Noun  & Top1 / 5 Act  & Top1 / 5 Verb  & Top1 / 5 Noun  & Top1 / 5 Act  & Top1 / 5 Verb  & Top1 / 5 Noun  \\\midrule
% \multirow{9}{*}{\rot{Fine-grained}} 
RGB &  8.23  /  25.01	& 25.42  /  60.53 &	22.08  /  45.71	& 9.02  /  27.60 &	27.20  /  64.48 & 	23.61  /  48.03	 & 0.13  /  0.18 & 9.44  /  25.00 & 8.28  /  24.83 \\
\midrule
Depth &  3.86  /  13.38 & 20.30  /  54.09 & 12.82  /  28.46 & 4.27  /  14.82 &  21.67  /  57.72 & 13.48  /  29.93 & 0.02  /  0.07 & 8.20  /  21.88 & 7.03  /  15.43 \\
R+D &  4.58  /  18.11  & 19.39  /  56.01 & 16.60  /  38.97 & 5.05  /  19.99 & 20.90  /  59.84 & 17.60  /  41.09 & 0.04  /  0.18 & 6.05  /  22.27 & 7.81  /  20.31 \\
\midrule
Hands    &     4.44  /  15.82                   &         20.72  /  56.92          &        15.20  /  28.06         &        4.93  /  17.57         &         22.25  /  60.95          &       16.67  /  30.44          &        0.00  /  0.00         &        6.95  /  20.70           &       1.99  /  6.62               \\
R+H & 10.37  /  29.30 & 29.00  /  65.75 &	25.09  /  49.45 & 11.39  /  32.26 & 31.17  /  70.08	& 26.63  /  52.02 & 0.13  /  0.29 & 9.44  /  26.82 & 11.26  /  26.32 \\
R+H+E & 6.94 / 21.31 & 24.74 / 60.77 & 19.40 / 41.42 & 7.61 / 23.38 & 26.39 / 64.55 & 20.61 / 43.47 & 0.09 / 0.28 & 9.78 / 26.48 & 8.43 / 22.77 \\
R+H+D & 7.21 / 21.33 & 25.58 / 60.80 & 18.92 / 39.77 & 7.96 / 23.52 & 27.44 / 65.08 & 20.04 / 41.85	& 0.08 / 0.23 & 9.15 / 23.05 & 8.98 / 21.36 \\
\midrule
R+H+E+D & 5.56 / 17.75 & 23.51 / 58.88 & 16.97 / 35.84 & 6.12 / 19.59 & 25.18 / 62.64 & 18.14 / 37.96 &	0.08 / 0.17 & 8.73 / 25.68 & 6.68 / 17.12 \\
R+H+E+D+I & 4.53 / 15.78 & 22.04 / 56.38 & 15.26 / 33.99 & 4.95 / 17.44 &  23.48 / 60.28 & 16.29 / 35.93 & 0.10 / 0.14 & 9.40 / 22.05 & 6.15 / 16.92\\ 
\midrule \midrule
RGB (Pt)      & 19.20  /  46.07       & 34.10  /  71.18     & 44.25  /  74.10     & 21.02  /  50.13       & 36.47  /  75.29     & 45.84  /  75.89     & 0.31  /  1.07         & 12.75  /  34.27     & 29.97  /  57.95 \\
\bottomrule
\end{tabular}}
\caption{\textbf{Action recognition benchmark results.} We report baseline results of (multimodal) TimeSformer~\cite{timesformer} models on \data. Here \texttt{R}, \texttt{D}, \texttt{H}, \texttt{I} denote RGB, depth, hands, and head pose (whose sensor source is similar as IMUs). The RGB model pre-trained on ImageNet (\texttt{RGB(Pt)}) achieves higher results than training from scratch. For different modalities, we notice that adding hands (\texttt{R+H}) can improve the prediction of \texttt{verbs} and lead to better results than the baseline \texttt{RGB} only model. Simply concatenating more sensors as inputs may not necessarily lead to improved performance. } \label{tab:action_recog} \vspace{-2mm}
\end{table*}

==> tabs/compare.tex <==
\begin{table*}[t]
\centering
\adjustbox{width=\linewidth}{
\begin{tabular}{@{}lm{0.2\linewidth}m{0.1\linewidth}ccccccc@{}}
Dataset          & Modalities                                                        & Scenarios               & \begin{tabular}[c]{@{}c@{}}Multi-people \\ interaction\end{tabular} & \begin{tabular}[c]{@{}c@{}}3D \\ sensors\end{tabular} & \begin{tabular}[c]{@{}c@{}}Length \\ in hours\end{tabular} & \begin{tabular}[c]{@{}c@{}}\# sensor \\ frames\end{tabular} & \# tasks & \# collectors & \begin{tabular}[c]{@{}c@{}}\# action \\ classes\end{tabular} \\ \midrule
H2O              &                                                                   &                         &                                                                     &                                                       &                                                            &                                                             &          &               &                                                              \\
EpicKitchen      & RGB                                                               & Kitchen                 & \xmark                                                               & \xmark                                                 & 100                                                        & 10M                                                         &          & 37            & 2513                                                         \\
Assembly101(Ego) & Gray-scale image, estimated 3D hand poses                         & Lab                     & \xmark                                                               & \xmark                                                 & 167                                                        &                                                             & 30       & 53            & 1380                                                         \\
Ego4D-Full       & RGB, text, audio                                                  & Wild                    & \cmark                                                               & \xmark                                                 & 3670                                                       &                                                             &          & 931           &                                                              \\
Ego4D-Forecast   & RGB, text, audio, hand bounding boxes                             & Wild                    & \cmark                                                               & \xmark                                                 & 110                                                        &                                                             &          &               &                                                              \\
Ego4D-EyeGaze    & RGB, text, audio, eye gaze                                        & Wild                    & \cmark                                                               & \xmark                                                 & 45                                                         &                                                             &          &               &                                                              \\
Ego4D-3DScan     & RGB, text,  audio, 3D Scan of room                                & Wild                    & \cmark                                                               & \cmark                                                 &                                                            &                                                             &          &               &                                                              \\
\midrule
\data (ours)      & RGB, text, audio, depth, 3D hand poses, eye gaze, head poses, IMU & Office, mechanical lab & \cmark                                                               & \cmark                                                 & 169                                                        &                                                             & 22       & 222           & 1677                                                         \\ \bottomrule
\end{tabular}}
\caption{Dataset comparison\xin{need to verif the numbers}}
\label{tab:dataset comparison}
\end{table*}

==> tabs/compare_3d.tex <==
\begin{table}[t]
\centering
\adjustbox{width=\linewidth}{
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|ccccccccc|ccc@{}}
\toprule
Dataset      
%& \rot{Images} & \rot{Text} & \rot{Audio} & \rot{Depth} & \rot{Eye Gaze} & \rot{Head Pose} & \rot{Hand Pose}  & \rot{IMU}        
& RGB & Depth & 
\begin{tabular}[c]{@{}c@{}}Head \\ pose\end{tabular} & \begin{tabular}[c]{@{}c@{}}Hand \\ pose\end{tabular}& 
\begin{tabular}[c]{@{}c@{}}Object \\ pose\end{tabular} & \begin{tabular}[c]{@{}c@{}}Eye \\ gaze\end{tabular} &
Audio  &  IMU    & \begin{tabular}[c]{@{}c@{}}Action \\ label\end{tabular}
& \# frames   \\ \midrule
FPHA~\cite{garcia2018first}              &   \cmark                                                                                                                            &    \cmark                                                   &    \xmark                                                          &             \cmark                                                &   \cmark            &      \xmark           &    \xmark        & \xmark  &\cmark                & 100k                                       \\
H2O~\cite{kwon2021h2o}              &     \cmark                                                                                                                            &    \cmark                                                   &            \cmark                                                &                     \cmark                                        &       \cmark        &       \xmark          &       \xmark    &       \xmark&            \cmark                    & 114k  \\% & &4                                  \\
EgoBody~\cite{egobody}              &    \cmark                                                                                                                                   &    \cmark                                                   &        \cmark                                                    &                \cmark                                             & \xmark          &         \cmark           & \xmark & \xmark & \xmark & 199k \\%& &36                                                              \\
Panoptic~\cite{Joo_2017_TPAMI}              &     \cmark                                                                                                                              &      \cmark                                                 &       \cmark                                                     &            \cmark                                                 &   \xmark       &    \xmark           &        & \xmark &\xmark          & 5.5 hours                                           \\
BABEL~\cite{BABEL:CVPR:2021}             &        \xmark                                                                                                                             &   \xmark                                                       &       \cmark                                                     &          \cmark                                                   &   \cmark        &          \xmark       &              \xmark  &  \xmark  & \cmark & 4.6m                                                 \\
BEHAVE~\cite{bhatnagar22behave}              &        \cmark                                                                                                                                 &                   \cmark                                           &             \cmark                                                      &          \cmark                                                          &     \cmark            &      \xmark            &     &  \xmark  &  \xmark  & 15k                                                     \\
Assembly101~\cite{assembly101} (ego) &\cmark\S
& \cmark & & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark
& 18 m        \\ %  &   1,425      & 53      \\
\midrule
\data (ours)     
& \cmark & \cmark & \cmark & \cmark& \xmark & \cmark & \cmark & \cmark & \cmark
& 18 m    \\  % &         2,243    & 222     \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Contemporary 3D datasets.} \data covers multi modalities. \S: monochrome videos.
}
\label{tab:egodataset comparison}
\end{table}

==> tabs/compare_bk.tex <==
\begin{table*}[t]
\centering
\adjustbox{width=\linewidth}{
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|cc|cccccccc|ccc@{}}
\toprule
Dataset        & Scenarios       &  Settings
%& \rot{Images} & \rot{Text} & \rot{Audio} & \rot{Depth} & \rot{Eye Gaze} & \rot{Head Pose} & \rot{Hand Pose}  & \rot{IMU}        
& RGB & Depth & 
\begin{tabular}[c]{@{}c@{}}Head \\ Pose\end{tabular} & \begin{tabular}[c]{@{}c@{}}Hand \\ pose\end{tabular} & \begin{tabular}[c]{@{}c@{}}Eye \\ gaze\end{tabular} &
Audio  &  IMU    & Text 
& \# hours  & \# sessions & \# collectors  \\ \midrule
Epic-Kitchen-100~\cite{epickitchen}      &  Kitchen       
& Unscripted activity
& \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark
& 100              &    700         & 37   \\
Assembly101~\cite{assembly101} (ego) &  Lab    
& Toy vehicle assembly
& \cmark\S & \xmark & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark
& 167            &   1,425      & 53      \\
Ego4D~\cite{ego4d} (full)      &  Wild        
& Daily-life activity
& \cmark  & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark
& 3,670           &   --   & 931        \\
Ego4D~\cite{ego4d} (with eye gaze)         & Wild    
& Daily-life activity
& \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \xmark & \cmark
& 45      &       572        &    --       \\
Ego4D~\cite{ego4d} (with IMU)         & Wild    
& Daily-life activity
& \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark
& 836      &       --        &    --       \\
Ego4D~\cite{ego4d} (with 3D scan)    & Wild       
& Daily-life activity
& \cmark & \cmark\ddag & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark
&    491              &     --          &      --     \\
\midrule
\data (ours)      & Office + Lab
& Assistive task completion
& \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark & \cmark
& 169       &         2,243    & 222     \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Contemporary multimodal egocentric datasets.} \data features an interactive assistive setting which is a unique addition to existing datasets.  \data also provides more synchronized modalities than previous datasets. Note that we list Ego4D subsets separately as the sensor modalities are disjoint subsets in the dataset. \data spans 169 hours and 2,243 sessions.  \S: monochrome videos; 
%\dag: hand bounding boxes; 
\ddag: 3D scans of the scenes.
\mahdicomment{Do we want to keep this table? As we discussed, although the table reports an accurate comparison, it might not be in our favor, as: 1) it could raise this concern that we are trying to show Ego-4D is not good. 2) Now our focus is more in emphasizing on interactive scenarios, than trying to say multi-modalities are important. Therefore, if we remove the modalities comparison, we are then showing we are much smaller compared to Ego-4D in terms of number of hours. }
}
\label{tab:dataset comparison}\vspace{-5mm}
\end{table*}

==> tabs/compare_egocentric.tex <==
\begin{table}[t]
\centering
\adjustbox{width=\linewidth}{
\setlength{\tabcolsep}{3pt}
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|cc|cccccccc|ccc@{}}
\toprule
Dataset        & Scenarios       &  Settings
& \# hours  & \# sessions & \# collectors  \\ \midrule
Epic-Kitchen-100~\cite{epickitchen}      &  Kitchen       
& Unscripted activity
& 100              &    700         & 37   \\
EGTEA~\cite{li2021eye}  
& Kitchen
&   Unscripted activity    &  28    &      86& 32   \\
Assembly101~\cite{assembly101} &  Lab    
& Toy vehicle assembly
& 167            &   1,425      & 53      \\
Ego4D~\cite{ego4d}      &  Wild        
& Daily-life activity
& 3,670           &   --   & 931        \\
\midrule
\data (ours)      & Office + Lab
&  \begin{tabular}[c]{@{}c@{}}Assistive task completion \\ with interaction\end{tabular} 
& 169       &         2,243    & 222     \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Contemporary egocentric datasets.} \data features an interactive assistive setting which is a unique addition to existing datasets.  \data has a large number of capture sessions and participants among the existing egocentric video datasets. \xin{needs updates}
}
\label{tab:egodataset_comparison} \vspace{-4mm}
\end{table}

==> tabs/compare_instruction.tex <==
\begin{table}[t]
\centering
\adjustbox{width=.75\linewidth}{
\setlength{\tabcolsep}{4pt}
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{@{}l|cc|cccccccc|ccc@{}}
\toprule
Dataset        & Real       &  Synthetic
& \# hours  & \# instructions \\ \midrule
ALFRED~\cite{ALFRED20}      &     
&  \cmark   

&               &             &    \\
Habitat~\cite{szot2021habitat} &      
&  \cmark   

&            &        &       \\
IGibson~\cite{li2021igibson}     &          
&  \cmark   

&           &     &         \\
BEHAVIOR~\cite{srivastava2022behavior}     &          
&  \cmark   

&           &     &         \\
\midrule
\data (ours)      &  \cmark   
& 

&        &            &      \\ 
\bottomrule
\end{tabular}}
\caption{\textbf{Contemporary instruction and interactive datasets.} \data has a unique position among embodied AI datasets by capturing real videos.
}
\label{tab:egodataset comparison}
\end{table}

==> tabs/intervention_0817.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{2pt} 
\adjustbox{width=\linewidth}{
\def\arraystretch{1.2}%  1 is the default, change whatever you need
\begin{tabular}{c|m{0.14\linewidth}|cc|cc|cc|cc}
\toprule
 &\multirow{2}{*}{Mods.} & \multicolumn{2}{c|}{Overall} & \multicolumn{2}{c|}{Confirm Action} & \multicolumn{2}{c|}{Correct Mistake} & \multicolumn{2}{c}{Follow-up} \\
& &Prec. & Recall & Prec. & Recall & Prec. & Recall & Prec. & Recall \\ \midrule
\multirow{5}{*}{\rotatebox{90}{Pretrained}} & RGB & 47.92 &	46.09 & 44.09 &	27.65 &	46.13 &	41.44 & 53.54 &	69.18\\
& Hands & 15.75	33.33 & 0 &	0 &	0 &	0 &	47.25 &	100 \\
& R+H & 48.08 &	47.06 &	43.64 & 32.21 &	46.63 &	44.67 &	53.95 &	64.3 \\
& R+E & 48.33 &	47.38 &	45.45 &	31.87 &	45.16 &	45.16 &	54.39 &	65.1\\
& R+H+E+H & 48.75 &	47.75 &	45.55 &	33.94 &	46.11 &	44.91 &	54.59 &	64.42 \\
\bottomrule
\end{tabular}} \caption{\textbf{Intervention type prediction results.} The classes in the intervention prediction benchmark are highly skewed. Here \texttt{E} refers to eye gaze. We can see the predictions of the baseline models (\ie, \texttt{RGB},\texttt{R+H}, \texttt{R+E}) favor predicting \texttt{follow-up instructions} while ignoring \texttt{correcting mistakes} (recall is 0). Training more modalities (\texttt{R+H+E}) alleviates this issue and even outperforms the pre-trained RGB model (\texttt{RGB(Pt)}) in overall precision.} \label{tab:intervention} \vspace{-4mm}
\end{table}


==> tabs/mistake.tex <==
\begin{table}[!htb]
    \begin{minipage}{.46\linewidth}
      \centering
      \setlength{\tabcolsep}{1pt} 
        \adjustbox{width=\linewidth}{
        \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{Mods.} & \multicolumn{2}{c}{Mistake} & \multicolumn{2}{c}{Correction} \\
         & Prec. & Rec. & Prec. & Rec. \\ \midrule
        % Random & 6.60 & 31.01 & 3.40 & 69.19 \\
        RGB & 0.00 & 0.00 & 0.00 & 0.00 \\
        R+H &  &  &  &  \\
        % R+D &  &  &  &  \\
        % R+H+D &  &  &  &  \\
        R+H+E &  &  &  &  \\
        \midrule
        RGB(Pt) & 7.16 & 19.95 & 4.75 & 22.22\\
        % RGB(Pt) & 11.04 & 7.93 & 0.00 & 0.00 \\
        \bottomrule
        \end{tabular}}
        \caption{Mistake detection}\label{tab:mistake_det}
    \end{minipage}~~
    \begin{minipage}{.46\linewidth}
    \setlength{\tabcolsep}{1pt} 
    \def\arraystretch{1.2}% 
    \adjustbox{width=\linewidth}{
    \begin{tabular}{lccc}
    \toprule
    \multirow{2}{*}{Mods.} & \multicolumn{3}{c}{Mean Error Dist.}\\ %& \multicolumn{3}{c}{Right Hand} \\
     & 0.5 sec & 1.0 sec & 1.5 sec\\ \midrule %& 0.5& 1.0 & 1.5 \\ \midrule
    Static-H & 9.80 & 13.94 & 16.63 \\
    H &  8.38 & 9.64 & 10.41 \\ 
    H+E & 8.01 & 9.26 & 9.97  \\
    \bottomrule
    \end{tabular}}\caption{3D Hand Pose Forecasting Benchmark. We report mean per joint position error for 0.5  1.0, 1.5 seconds, static hand given from last frame of the input \textbf{Static-H}, and  for seq2seq~\cite{sutskever2014sequence} model trained using hands only \textbf{H}, hands and eye gaze \textbf{H+E}.}\label{tab:hand_pose}
    \end{minipage} 
\end{table}
